Cross-Correlation Redshift Calibration Without Spectroscopic Calibration Samples in DES Science Verification Data

Galaxy cross-correlations with high-fidelity redshift samples hold the potential to precisely calibrate systematic photometric redshift uncertainties arising from the unavailability of complete and representative training and validation samples of galaxies. However, application of this technique in the Dark Energy Survey (DES) is hampered by the relatively low number density, small area, and modest redshift overlap between photometric and spectroscopic samples. We propose instead using photometric catalogs with reliable photometric redshifts for photo-z calibration via cross-correlations. We verify the viability of our proposal using redMaPPer clusters from the Sloan Digital Sky Survey (SDSS) to successfully recover the redshift distribution of SDSS spectroscopic galaxies. We demonstrate how to combine photo-z with cross-correlation data to calibrate photometric redshift biases while marginalizing over possible clustering bias evolution in either the calibration or unknown photometric samples. We apply our method to DES Science Verification (DES SV) data in order to constrain the photometric redshift distribution of a galaxy sample selected for weak lensing studies, constraining the mean of the tomographic redshift distributions to a statistical uncertainty of $\Delta z \sim \pm 0.01$. We forecast that our proposal can in principle control photometric redshift uncertainties in DES weak lensing experiments at a level near the intrinsic statistical noise of the experiment over the range of redshifts where redMaPPer clusters are available. Our results provide strong motivation to launch a program to fully characterize the systematic errors from bias evolution and photo-z shapes in our calibration procedure.

==> dessv-photo-z (2)/acknowledgments.tex <==
CPD would like to acknowledge Enrique Gaztanaga, Marco Gatti, Pauline Vielzeuf, Ross Cawthon, \`{A}lex Alarc\'{o}n for many fruitful conversations. He would also like to thank Ben Hoyle, Huan Lin, Ramon Miquel, and Michael Troxel for their many suggestions, which tremendously improved this paper. This work is partially supported by the Northern California Chapter of the ARCS Foundation, as well as by the U.S. Department of Energy under contract number DE-AC02-76-SF00515.
ER is supported by DOE grant DE-SC0015975 and by the Sloan Foundation, grant FG-2016-6443.

Funding for the DES Projects has been provided by the U.S. Department of Energy, the U.S. National Science Foundation, the Ministry of Science and Education of Spain, 
the Science and Technology Facilities Council of the United Kingdom, the Higher Education Funding Council for England, the National Center for Supercomputing 
Applications at the University of Illinois at Urbana-Champaign, the Kavli Institute of Cosmological Physics at the University of Chicago, 
the Center for Cosmology and Astro-Particle Physics at the Ohio State University,
the Mitchell Institute for Fundamental Physics and Astronomy at Texas A\&M University, Financiadora de Estudos e Projetos, 
Funda{\c c}{\~a}o Carlos Chagas Filho de Amparo {\`a} Pesquisa do Estado do Rio de Janeiro, Conselho Nacional de Desenvolvimento Cient{\'i}fico e Tecnol{\'o}gico and 
the Minist{\'e}rio da Ci{\^e}ncia, Tecnologia e Inova{\c c}{\~a}o, the Deutsche Forschungsgemeinschaft and the Collaborating Institutions in the Dark Energy Survey. 

The Collaborating Institutions are Argonne National Laboratory, the University of California at Santa Cruz, the University of Cambridge, Centro de Investigaciones Energ{\'e}ticas, 
Medioambientales y Tecnol{\'o}gicas-Madrid, the University of Chicago, University College London, the DES-Brazil Consortium, the University of Edinburgh, 
the Eidgen{\"o}ssische Technische Hochschule (ETH) Z{\"u}rich, 
Fermi National Accelerator Laboratory, the University of Illinois at Urbana-Champaign, the Institut de Ci{\`e}ncies de l'Espai (IEEC/CSIC), 
the Institut de F{\'i}sica d'Altes Energies, Lawrence Berkeley National Laboratory, the Ludwig-Maximilians Universit{\"a}t M{\"u}nchen and the associated Excellence Cluster Universe, 
the University of Michigan, the National Optical Astronomy Observatory, the University of Nottingham, The Ohio State University, the University of Pennsylvania, the University of Portsmouth, 
SLAC National Accelerator Laboratory, Stanford University, the University of Sussex, Texas A\&M University, and the OzDES Membership Consortium.

The DES data management system is supported by the National Science Foundation under Grant Number AST-1138766 and AST-1536171.
The DES participants from Spanish institutions are partially supported by MINECO under grants AYA2015-71825, ESP2015-88861, FPA2015-68048, SEV-2012-0234, SEV-2012-0249, and MDM-2015-0509, 
some of which include ERDF funds from the European Union. IFAE is partially funded by the CERCA program of the Generalitat de Catalunya.

We are grateful for the extraordinary contributions of our CTIO colleagues and the DECam Construction, Commissioning and Science Verification
teams in achieving the excellent instrument and telescope conditions that have made this work possible.  The success of this project also 
relies critically on the expertise and dedication of the DES Data Management group.


==> dessv-photo-z (2)/addresses.tex <==
\def\kipac{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, 452 Lomita Mall, Stanford, CA 94035, USA}
\def\slac{Department of Particle Physics and Astrophysics, SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, CA 94025, USA}
\def\stanford{Department of Physics, Stanford University, 382 Via Pueblo, Stanford, CA 94305, USA}

\def\uofa{Department of Physics, University of Arizona, Tucson, AZ 85721, USA}

\def\cpdemail{\tt cpd@stanford.edu}


==> dessv-photo-z (2)/affiliations.tex <==

$^{1}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{2}$ Institute of Space Sciences, IEEC-CSIC, Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{3}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{4}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{5}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{6}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{7}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{8}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{9}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{10}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{11}$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile\\
$^{12}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{13}$ Department of Physics and Electronics, Rhodes University, PO Box 94, Grahamstown, 6140, South Africa\\
$^{14}$ LSST, 933 North Cherry Avenue, Tucson, AZ 85721, USA\\
$^{15}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{16}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{17}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{18}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{19}$ Department of Astronomy, University of Illinois, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{20}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{21}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{22}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{23}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{24}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{25}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{26}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{27}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{28}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$^{29}$ Astronomy Department, University of Washington, Box 351580, Seattle, WA 98195, USA\\
$^{30}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{31}$ Australian Astronomical Observatory, North Ryde, NSW 2113, Australia\\
$^{32}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$^{33}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{34}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{35}$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA\\
$^{36}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{37}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{38}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{39}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{40}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{41}$ Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil\\
$^{42}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{43}$ Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{44}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\

==> dessv-photo-z (2)/authors.tex <==
% Author list file generated with: mkauthlist 1.2.2 
% mkauthlist -j mnras DES-2016-0206_author_list.csv DES-2016-0206.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
C.~Davis$^{1}$\thanks{E-mail: cpd@stanford.edu (CPD) },
E.~Rozo$^{8}$,
A.~Roodman$^{1,7}$,
A.~Alarcon$^{2}$,
R.~Cawthon$^{3}$,
M.~Gatti$^{4}$,
H.~Lin$^{5}$,
R.~Miquel$^{6,4}$,
E.~S.~Rykoff$^{1,7}$,
M.~A.~Troxel$^{9,10}$,
P.~Vielzeuf$^{4}$,
T. M. C.~Abbott$^{11}$,
F.~B.~Abdalla$^{12,13}$,
S.~Allam$^{5}$,
J.~Annis$^{5}$,
K.~Bechtol$^{14}$,
A.~Benoit-L{\'e}vy$^{15,12,16}$,
E.~Bertin$^{15,16}$,
D.~Brooks$^{12}$,
E.~Buckley-Geer$^{5}$,
D.~L.~Burke$^{1,7}$,
A. Carnero Rosell$^{17,18}$,
M.~Carrasco~Kind$^{19,20}$,
J.~Carretero$^{4}$,
F.~J.~Castander$^{2}$,
M.~Crocce$^{2}$,
C.~E.~Cunha$^{1}$,
C.~B.~D'Andrea$^{21}$,
L.~N.~da Costa$^{17,18}$,
S.~Desai$^{22}$,
H.~T.~Diehl$^{5}$,
P.~Doel$^{12}$,
A.~Drlica-Wagner$^{5}$,
A.~Fausti Neto$^{17}$,
B.~Flaugher$^{5}$,
P.~Fosalba$^{2}$,
J.~Frieman$^{5,3}$,
J.~Garc\'ia-Bellido$^{23}$,
E.~Gaztanaga$^{2}$,
D.~W.~Gerdes$^{24,25}$,
T.~Giannantonio$^{26,27,28}$,
D.~Gruen$^{1,7}$,
R.~A.~Gruendl$^{19,20}$,
G.~Gutierrez$^{5}$,
K.~Honscheid$^{9,10}$,
B.~Jain$^{21}$,
D.~J.~James$^{29,11}$,
T.~Jeltema$^{30}$,
E.~Krause$^{1}$,
K.~Kuehn$^{31}$,
S.~Kuhlmann$^{32}$,
N.~Kuropatkin$^{5}$,
O.~Lahav$^{12}$,
T.~S.~Li$^{5}$,
M.~Lima$^{33,17}$,
M.~March$^{21}$,
J.~L.~Marshall$^{34}$,
P.~Martini$^{9,35}$,
P.~Melchior$^{36}$,
R.~L.~C.~Ogando$^{17,18}$,
A.~A.~Plazas$^{37}$,
A.~K.~Romer$^{38}$,
E.~Sanchez$^{39}$,
V.~Scarpine$^{5}$,
R.~Schindler$^{7}$,
M.~Schubnell$^{25}$,
I.~Sevilla-Noarbe$^{39}$,
M.~Smith$^{40}$,
M.~Soares-Santos$^{5}$,
F.~Sobreira$^{41,17}$,
E.~Suchyta$^{42}$,
M.~E.~C.~Swanson$^{20}$,
G.~Tarle$^{25}$,
D.~Thomas$^{43}$,
V.~Vikram$^{32}$,
A.~R.~Walker$^{11}$,
R.~H.~Wechsler$^{44,1,7}$
\begin{center} (DES Collaboration) \end{center}
}
}
\vspace{0.4cm}
